Contrastive Multiview Coding with Electro-optics for SAR Semantic Segmentation

In the training of deep learning models, how the model parameters are initialized greatly affects the model performance, sample efficiency, and convergence speed. Representation learning for model initialization has recently been actively studied in the remote sensing field. In particular, the appearance characteristics of the imagery obtained using the a synthetic aperture radar (SAR) sensor are quite different from those of general electro-optical (EO) images, and thus representation learning is even more important in remote sensing domain. Motivated from contrastive multiview coding, we propose multi-modal representation learning for SAR semantic segmentation. Unlike previous studies, our method jointly uses EO imagery, SAR imagery, and a label mask. Several experiments show that our approach is superior to the existing methods in model performance, sample efficiency, and convergence speed.

==> table_epoch.tex <==

\begin{table}[]
    \centering
    \begin{tabular}{l|ccccc} \\
    & \multicolumn{5}{c}{Epoch} \\
    Model & 5 & 10 & 15 & 20 & 25 \\
    \toprule
    (1) & 0.9473 & 0.9537 & 0.9573 & 0.9588 & 0.9594 \\
    (2) & 0.9317 & 0.9583 & 0.9631 & 0.9650 & 0.9658 \\
    (3) & 0.9532 & 0.9607 & 0.9650 & 0.9668 & 0.9678 \\
    (4) & 0.9317 & 0.9687 & 0.9709 & 0.9720 & 0.9724 \\
    (5) & 0.9696 & 0.9722 & 0.9733 & 0.9740 & 0.9742 \\
    (6) & $\bm{0.9692}$ & $\bm{0.9721}$ & $\bm{0.9736}$ & $\bm{0.9743}$ & $\bm{0.9745}$ \\
    \midrule
    \end{tabular}
    \caption{This table shows the pixel accuracy of each checkpoint over the training epochs. }
    \label{tab:Accuracy Table}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{l|ccccc} \\
    & \multicolumn{5}{c}{Epoch} \\
    Model & 5 & 10 & 15 & 20 & 25 \\
    \toprule
    (1) & 0.3428 & 0.4465 & 0.4784 & 0.5038 & 0.5126 \\
    (2) & 0.0000 & 0.5174 & 0.5340 & 0.5655 & 0.5818 \\
    (3) & 0.4202 & 0.5299 & 0.5568 & 0.5874 & 0.5996 \\
    (4) & 0.0000 & 0.6122 & 0.6368 & 0.6479 & 0.6517 \\
    (5) & $\bm{0.6179}$ & $\bm{0.6444}$ & 0.6586 & 0.6688 & 0.6708 \\
    (6) & 0.6073 & 0.6432 & $\bm{0.6607}$ & $\bm{0.6707}$ & $\bm{0.6738}$ \\
    \midrule
    \end{tabular}
    \caption{This table shows the IoU of each checkpoint over the training epochs.}
    \label{tab:IoU Table}
\end{table}

==> table_representation.tex <==
\begin{table}[]
    \centering
    \begin{adjustbox}{width=0.32\textwidth}
    \begin{tabular}{c|c|c|c|c}
    \toprule
    {\color{blue-violet}Pretrain Source} & ImagNet & EO & SAR & Seg Map \\
    \midrule
    (1) &            &            &            &  \\
    (2) & \checkmark &            &            &  \\
    (3) &            &            & \checkmark &  \\
    (4) &            & \checkmark & \checkmark &  \\
    (5) &            &            & \checkmark & \checkmark \\
    (6) &            & \checkmark & \checkmark & \checkmark \\
    \midrule
    \end{tabular}
    \end{adjustbox}
    \caption{\color{blue} This table shows that what conditions each backbone performed contrastive multiview coding. Model (1) refers to a model that has been randomly initialized using He's method \cite{he2015delving} without any pretraining. Model (2) indicates the ImageNet-pretrained model. Similar to several other works\cite{kang2020deep,manas2021seasonal}, model (3) refers to contrastive learning (Equation \ref{eq:cl}) on SAR images. Checkmarks in other models indicate the type of image used in contrastive multiview coding.}
    \label{tab:Condition Table}
\end{table}
